Simulating Native Speaker Shadowing for Nonnative Speech Assessment with Latent Speech Representations

Evaluating speech intelligibility is a critical task in computer-aided language learning systems. Traditional methods often rely on word error rates (WER) provided by automatic speech recognition (ASR) as intelligibility scores. However, this approach has significant limitations due to notable differences between human speech recognition (HSR) and ASR. A promising alternative is to involve a native (L1) speaker in shadowing what nonnative (L2) speakers say. Breakdowns or mispronunciations in the L1 speaker's shadowing utterance can serve as indicators for assessing L2 speech intelligibility. In this study, we propose a speech generation system that simulates the L1 shadowing process using voice conversion (VC) techniques and latent speech representations. Our experimental results demonstrate that this method effectively replicates the L1 shadowing process, offering an innovative tool to evaluate L2 speech intelligibility. Notably, systems that utilize self-supervised speech representations (S3R) show a higher degree of similarity to real L1 shadowing utterances in both linguistic accuracy and naturalness.

==> fig/l1shadowingl2_w_lb.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.8\textwidth]{fig/l1shadowingl2_w_lb.png}
	\captionof{figure}{The proposed shadowing technique aims to identify unintelligible parts in an L2 speaker's reading aloud utterances ($L2_{R}$). In this approach, $L1_{S1}$ represents a native speaker’s initial shadowing, while $L1_{SS}$ denotes the script-shadowing by the native speaker.
By calculating the distance between $L1_{S1}$ and $L1_{SS}$, it is possible to pinpoint the native speaker's listening breakdowns, which correspond to the unintelligible parts in the $L2_{R}$ as well.}
	\label{fig:l1shadowingl2_w_lb}
\vspace{-5mm}
\end{figure*}

==> fig/vs_concept.tex <==
\begin{figure}[t]
%     \vspace{-1cm}
	\centering
	\includegraphics[width=\columnwidth]{fig/vs_concept.png}
    \vspace{-5mm}
 	\captionof{figure}{The concept of the virtual shadower, which simulates the shadowing behaviors of an L1 rater hearing a given L2 speech for the first time. Stuttering or inarticulate production of speech may occur due to listening disfluencies.}
 	\label{fig:vs_concept}
      \vspace{-5mm}
\end{figure}

==> nat.tex <==
\begin{table}
  \centering
\caption{Speech naturalness evaluation results for L1-shadowing-L2 System: all systems use $L2_{R}$ and $L1_{S1}$ as source and target, respectively.}
  \begin{tabular}{@{}cccc}
  \toprule
  Description&Source feat.&Target feat.&UTMOS$\uparrow$\\
  \midrule
Baseline A)&PPG-BNF&Mel.&3.40\\
 Baseline B)& PPG-BNF& PPG-BNF&3.58\\
\midrule
 Method A)& HuBERT& Mel.&3.70 \\
 Method B)& HuBERT& PPG-BNF&3.93 \\
\midrule
 Method C)& HuBERT& Mel.&3.44 \\
 Method C)& HuBERT& PPG-BNF&3.91 \\
\midrule
 Method D)& HuBERT& Mel.&3.77 \\
 Method D)& HuBERT& PPG-BNF&\textbf{3.96} \\
\bottomrule
\end{tabular}

\label{tab:vs_nat}
\end{table}

==> speechbertscore.tex <==
\begin{table}
  \centering
\caption{Speech naturalness evaluation results for L1-shadowing-L2 System: all systems use $L2_{R}$ and $L1_{S1}$ as source and target, respectively.}
  \begin{tabular}{@{}cccc@{}}
  \toprule
  Description&Source feat.&Target feat.&SpeechBERTScore$\uparrow$ \\
  \midrule
Baseline A)&PPG-BNF&Mel.&0.6437 \\
 Baseline B)& PPG-BNF& PPG-BNF&0.6716 \\
\midrule
 Method A)& HuBERT& Mel.&0.7424 \\
 Method B)& HuBERT& PPG-BNF&0.7568 \\
\midrule
 Method C)& HuBERT& Mel.&0.6927 \\
 Method C)& HuBERT& PPG-BNF&0.7429 \\
\midrule
 Method D)& HuBERT& Mel.&0.7579 \\
 Method D)& HuBERT& PPG-BNF&\textbf{0.7627} \\
\bottomrule
\end{tabular}

\label{tab:vs_nat}
\end{table}



\begin{table*}
  \centering
\caption{}
  \begin{tabular}{@{}cccccccccc@{}}
  \toprule
  Description& Input     &Source    &Source feat.& Target    &Target feat.& S1-CER $\downarrow$ & S1-WER$\downarrow$ &BERT$\uparrow$ &SpeechBERT$\uparrow$ \\
  \midrule
& $L1_{S1}$   &-   &-   & -  &-   & - & -   &-&- \\
& $L1_{SS}$   &-   &-   & -  &-   & 6.74& 12.46&0.971&0.840 \\
& $L2_{R}$        &-   &-   & -  &-   & 12.70& 24.25&0.939&0.618 \\
  \midrule    
ANA-SYN& $L1_{S1}$   &$L1_{spk}$       &PPG-BNF& $L1_{spk}$     &-   & 2.23& 5.82&0.984&0.8913\\
& $L1_{SS}$   &$L1_{spk}$       &PPG-BNF& $L1_{spk}$     &-   & 7.54& 13.72&0.967&0.8081\\
& $L2_{R}$        &$L2_{spk}$       &PPG-BNF& $L2_{spk}$     &-   & 22.94& 40.26&0.898&0.6045\\
& $L2_{R}$        &$L2_{spk}$       &PPG-BNF& $L1_{spk}$     &-   & 23.24& 40.77&0.894
&0.4840\\
\midrule
Baseline A)& $L2_{R}$   &$L2_{R}$&PPG-BNF& $L1_{S1}$&Mel.& 21.66& 37.73&0.903&0.6716 \\
& $L2_{R}$   &$L2_{R}$&PPG-BNF& $L1_{SS}$&Mel.& 22.54& 39.36&0.899&0.7212 \\
& $L2_{R}$   & $L1_{SS}$& PPG-BNF& $L1_{S1}$& Mel.& 21.66& 37.73& 0.903&0.6716 \\
  \midrule
Baseline B)& $L2_{R}$   & $L2_{R}$&PPG-BNF&  $L1_{S1}$&PPG-BNF& 38.07&   58.69&0.862&0.6437 \\
& $L2_{R}$   & $L2_{R}$&PPG-BNF&  $L1_{SS}$&PPG-BNF& 28.60&   46.77&0.881&0.6882 \\
 & $L2_{R}$   & $L1_{SS}$& PPG-BNF& $L1_{S1}$& PPG-BNF& 27.45& 47.68& 0.882&0.6716 \\
\midrule
 Method A)& $L2_{R}$   & $L2_{R}$   & HuBERT& $L1_{S1}$& Mel.& 18.02& 31.82& 0.919&0.7424 \\
 Method A)& $L2_{R}$   & $L2_{R}$   & HuBERT& $L1_{SS}$& Mel.& \textbf{16.31}& \textbf{28.53}& \textbf{0.926}&0.7536 \\
 Method B)& $L2_{R}$   & $L2_{R}$   & HuBERT& $L1_{S1}$& PPG-BNF& 19.19& 33.53& 0.912&0.7568 \\
 Method B)& $L2_{R}$   & $L2_{R}$   & HuBERT& $L1_{SS}$& PPG-BNF& 17.79& 31.67& 0.921&\textbf{0.7651} \\
\midrule
 Method C)& $L2_{R}$   & $L2_{R}$   & HuBERT& $L1_{S1}$& Mel.& 25.80& 43.19& 0.891&0.6927 \\
 Method C)& $L2_{R}$   & $L2_{R}$   & HuBERT& $L1_{S1}$& PPG-BNF& 20.70& 35.83& 0.912&0.7429 \\
\midrule
 Method D)& $L2_{R}$   & $L2_{R}$   & HuBERT& $L1_{S1}$& Mel.& 16.59& 29.74& 0.924&0.7579 \\
Method D)& $L2_{R}$   & $L2_{R}$   & HuBERT& $L1_{S1}$& PPG-BNF& 18.33& 32.12& 0.919&0.7627 \\
\bottomrule
\end{tabular}

\label{tab:vs_cer_wer}
\end{table*}


